Robust Multi-Robot Trajectory Optimization Using Alternating Direction Method of Multiplier

We propose a variant of alternating direction method of multiplier (ADMM) to solve constrained trajectory optimization problems. Our ADMM framework breaks a joint optimization into small sub-problems, leading to a low iteration cost and decentralized parameter updates. Starting from a collision-free initial trajectory, our method inherits the theoretical properties of primal interior point method (P-IPM), i.e., guaranteed collision avoidance and homotopy preservation throughout optimization, while being orders of magnitude faster. We have analyzed the convergence and evaluated our method for time-optimal multi-UAV trajectory optimizations and simultaneous goal-reaching of multiple robot arms, where we take into consider kinematics-, dynamics-limits, and homotopy-preserving collision constraints. Our method highlights an order of magnitude's speedup, while generating trajectories of comparable qualities as state-of-the-art P-IPM solver.

==> LipschitzDT.tex <==
\section{\label{sec:propertyDT}Lipschitz Continuity}
In the following derivation, we use shorthand notation $\tilde{V}_i=\TWO{\bar{V}_i}{\sqrt{\epsilon}}$ and $\tilde{A}_i=\TWO{\bar{A}_i}{\epsilon}$.

\begin{IEEEproof}[Proof of \prettyref{lem:contDeltaT}]
$\Delta t(\bar{X}_i)$ is differentiable due to \autocite[Theorem~4.2]{still2018lectures}. We can evaluate the gradient of $\Delta t(\bar{X}_i)$ via the implicit function theorem as:
\footnotesize
\begin{align*}
\FPP{\Delta t}{\bar{X}_i}=&
\left[\sum_i\frac{v_\text{max}^2}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2}+
\sum_i\frac{2a_\text{max}^2\Delta t^2+2a_\text{max}\|\tilde{A}_i\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\right]^{-1}\\
&\left[\frac{v_\text{max}\dot{I}^T\tilde{V}_i}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2\|\tilde{V}_i\|}+
\frac{2a_\text{max}\Delta t\ddot{I}^T\tilde{A}_i}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2\|\tilde{A}_i\|}\right].
\end{align*}
\normalsize
The smoothness follows from the composite function form of $\Delta t/\bar{X}_i$ and the positivity of denominator.
\end{IEEEproof}
\begin{lemma}
\label{lem:DeltaTA}
There exists $L_{\Delta t}^{1,2}$ such that $\FPPR{\Delta t(\bar{X}_i)}{\bar{X}_i}\leq L_{\Delta t}^1/L_{\Delta t}^2$.
\end{lemma}
\begin{IEEEproof}
At the global minima, we have:
\begin{equation*}
\frac{w}{\gamma}=\sum_i\frac{v_\text{max}}{v_\text{max}\Delta t-\|\tilde{V}_i\|}+
\sum_i\frac{2a_\text{max}\Delta t}{a_\text{max}\Delta t^2-\|\tilde{A}_i\|},
\end{equation*}
from which we immediately have:
\begin{align*}
&\frac{v_\text{max}}{v_\text{max}\Delta t-\|\tilde{V}_i\|}\leq\frac{w}{\gamma} \quad
\frac{2a_\text{max}\Delta t}{a_\text{max}\Delta t^2-\|\tilde{A}_i\|}\leq\frac{w}{\gamma}\\
&\frac{2}{\sqrt{\Delta t^2-\|\tilde{A}_i\|/a_\text{max}}}\leq\frac{2\Delta t}{\Delta t^2-\|\tilde{A}_i\|/a_\text{max}}\leq\frac{w}{\gamma}\\
\Rightarrow&\frac{1}{\Delta t^2-\|\tilde{A}_i\|/a_\text{max}}\leq\frac{w^2}{4\gamma^2},
\labelthis{eq:boundDTDX}
\end{align*}
and by Jensen's inequality, we have:
\small
\begin{align*}
&\left[\sum_i\frac{v_\text{max}^2}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2}+\sum_i\frac{4a_\text{max}^2\Delta t^2}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\right]\labelthis{eq:Jensen}\\
\geq&\frac{1}{\sum_i2}\left[\sum_i\frac{v_\text{max}}{v_\text{max}\Delta t-\|\tilde{V}_i\|}+
\sum_i\frac{2a_\text{max}\Delta t}{a_\text{max}\Delta t^2-\|\tilde{A}_i\|}\right]^2
=\frac{w^2}{\gamma^2\sum_i2}.
\end{align*}
\normalsize
We can then plug \prettyref{eq:Jensen} into the denominator and \prettyref{eq:boundDTDX} into the numerator of $\FPPR{\Delta t(\bar{X}_i)}{\bar{X}_i}$ to bound its norm:
\small
\begin{align*}
&\left\|\FPP{\Delta t(\bar{X}_i)}{\bar{X}_i}\right\|\leq\left[\frac{w^2}{\gamma^2\sum_i1}\right]^{-1}\\
&\left[\frac{w^2}{v_\text{max}\gamma^2}\fmax{s\in[0,1]}\|\dot{I}(s)\|+\frac{w^3}{4a_\text{max}\gamma^3}\fmax{s\in[0,1]}\|\ddot{I}(s)\|\right]\triangleq\frac{L_{\Delta t}^1}{L_{\Delta t}^2},
\end{align*}
\normalsize
which involves two bounds for the numerator and denominator, respectively.
\end{IEEEproof}
\begin{lemma}
\label{lem:DeltaTB}
There exists constants $L_{\Delta t}^{3,4}$ such that:
\small
\begin{align*}
&\left\|\FPP{}{\bar{X}_j}\left[\sum_i\frac{v_\text{max}^2}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2}+
\sum_i\frac{2a_\text{max}^2\Delta t^2+2a_\text{max}\|\tilde{A}_i\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\right]\right\|\\
\leq&L_{\Delta t}^3+L_{\Delta t}^4\frac{2a_\text{max}\|\tilde{A}_j\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_j\|)^2}.
\end{align*}
\normalsize
\end{lemma}
\begin{IEEEproof}
We show that the following gradient of the first term is bounded:
\begin{align*}
&\left\|\FPP{}{\bar{X}_j}\frac{v_\text{max}^2}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2}\right\|
=\left\|\frac{2v_\text{max}^2(v_\text{max}\FPP{\Delta t}{\bar{X}_j}-\frac{\dot{I}^T\tilde{V}_i}{\|\tilde{V}_i\|}\delta_{ij})}
{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^3}\right\|\\
\leq&\frac{2w^3}{\gamma^3}\frac{L_{\Delta t}^1}{L_{\Delta t}^2}+\frac{2w^3}{v_\text{max}\gamma^3}\fmax{s\in[0,1]}\|\dot{I}(s)\|\delta_{ij}.
\end{align*}
The following bounded gradient of the second term holds:
\tiny
\begin{align*}
&\left\|\FPP{}{\bar{X}_j}\frac{2a_\text{max}^2\Delta t^2+2a_\text{max}\|\tilde{A}_i\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\right\|\\
\leq&\left\|\frac{4a_\text{max}^2\Delta t\FPP{\Delta t}{\bar{X}_j}+2a_\text{max}\frac{\ddot{I}^T\tilde{A}_i}{\|\tilde{A}_i\|}\delta_{ij}}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\right\|+\\
&\left\|\frac{4a_\text{max}^2\Delta t^2+4a_\text{max}\|\tilde{A}_i\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^3}(2a_\text{max}\Delta t\FPP{\Delta t}{\bar{X}_j}-\frac{\ddot{I}^T\tilde{A}_i}{\|\tilde{A}_i\|}\delta_{ij})\right\|\\
=&\left\|\frac{4a_\text{max}^2\Delta t\FPP{\Delta t}{\bar{X}_j}+2a_\text{max}\frac{\ddot{I}^T\tilde{A}_i}{\|\tilde{A}_i\|}\delta_{ij}}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\right\|+\\
&\left\|\frac{8a_\text{max}^3\Delta t^3\FPP{\Delta t}{\bar{X}_j}+8a_\text{max}^2\Delta t\|\tilde{A}_i\|\FPP{\Delta t}{\bar{X}_j}-4a_\text{max}^2\Delta t^2\frac{\ddot{I}^T\tilde{A}_i}{\|\tilde{A}_i\|}\delta_{ij}-4a_\text{max}\ddot{I}^T\tilde{A}_i\delta_{ij}}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^3}\right\|\\
\leq&\frac{w^3}{2\gamma^3}\frac{L_{\Delta t}^1}{L_{\Delta t}^2}+\frac{w^4}{8a_\text{max}\gamma^4}\fmax{s\in[0,1]}\|\ddot{I}(s)\|\delta_{ij}+\\
&\frac{w^3}{\gamma^3}\frac{L_{\Delta t}^1}{L_{\Delta t}^2}+
\frac{2w}{\gamma}\frac{L_{\Delta t}^1}{L_{\Delta t}^2}\frac{2a_\text{max}\|\tilde{A}_i\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}+\frac{w^4}{4a_\text{max}\gamma^4}\fmax{s\in[0,1]}\|\ddot{I}(s)\|\delta_{ij}+\\
&\frac{w^2}{2a_\text{max}\gamma^2}\fmax{s\in[0,1]}\|\ddot{I}(s)\|\frac{2a_\text{max}\|\tilde{A}_i\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2}\delta_{ij}.
\end{align*}
\normalsize
The result follows by combining the above two equations and replacing constants.
\end{IEEEproof}
\begin{lemma}
\label{lem:DeltaTC}
There exists constants $L_{\Delta t}^5$ such that:
\footnotesize
\begin{align*}
\left\|\FPP{}{\bar{X}_j}\left[\frac{v_\text{max}\dot{I}^T\tilde{V}_i}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2\|\tilde{V}_i\|}+
\frac{2a_\text{max}\Delta t\ddot{I}^T\tilde{A}_i}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2\|\tilde{A}_i\|}\right]\right\|_F\leq L_{\Delta t}^5.
\end{align*}
\normalsize
\end{lemma}
\begin{IEEEproof}
We show the following gradient of first term is bounded:
\footnotesize
\begin{align*}
&\left\|\FPP{}{\bar{X}_j}\frac{v_\text{max}\dot{I}^T\tilde{V}_i}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2\|\tilde{V}_i\|}\right\|_F=
\left\|\frac{v_\text{max}\dot{I}^T\dot{I}\delta_{ij}}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2\|\tilde{V}_i\|}\right\|_F+\\
&\left\|\frac{v_\text{max}\dot{I}^T\tilde{V}_i\tilde{V}_i^T\dot{I}\delta_{ij}}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^2\|\tilde{V}_i\|^2}\right\|_F+
\left\|\frac{2v_\text{max}\dot{I}^T\tilde{V}_i(v_\text{max}\FPP{\Delta t}{\bar{X}_j}-\frac{\dot{I}^T\tilde{V}_i}{\|\tilde{V}_i\|}\delta_{ij})^T}{(v_\text{max}\Delta t-\|\tilde{V}_i\|)^3\|\tilde{V}_i\|}\right\|_F\\
\leq&\frac{w^2}{v_\text{max}\gamma^2\sqrt{\epsilon}}\fmax{s\in[0,1]}\|\dot{I}(s)\|^2\delta_{ij}+
\frac{w^2}{v_\text{max}\gamma^2}\fmax{s\in[0,1]}\|\dot{I}(s)\|^2\delta_{ij}+\\
&\frac{2w^3}{v_\text{max}\gamma^3}\frac{L_{\Delta t}^1}{L_{\Delta t}^2}\fmax{s\in[0,1]}\|\dot{I}(s)\|+
\frac{2w^3}{v_\text{max}^2\gamma^3}\fmax{s\in[0,1]}\|\dot{I}(s)\|^2\delta_{ij}.
\end{align*}
\normalsize
We then show the following gradient of second term is also bounded:
\footnotesize
\begin{align*}
&\left\|\FPP{}{\bar{X}_j}\frac{2a_\text{max}\Delta t\ddot{I}^T\tilde{A}_i}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2\|\tilde{A}_i\|}\right\|_F=\left\|\frac{2a_\text{max}\Delta t\ddot{I}^T\ddot{I}\delta_{ij}}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2\|\tilde{A}_i\|}\right\|_F+\\
&\left\|\frac{2a_\text{max}\Delta t\ddot{I}^T\tilde{A}_i\tilde{A}_i^T\ddot{I}\delta_{ij}}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2\|\tilde{A}_i\|^2}\right\|_F+\\
&\left\|\frac{4a_\text{max}\Delta t\ddot{I}^T\tilde{A}_i(2a_\text{max}\Delta t\FPP{\Delta t}{\bar{X}_j}-\frac{\ddot{I}^T\tilde{A}_i}{\|\tilde{A}_i\|}\delta_{ij})}{(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^3\|\tilde{A}_i\|}\right\|_F\\
\leq&\frac{w^3}{4a_\text{max}\gamma^3\epsilon}\fmax{s\in[0,1]}\|\ddot{I}(s)\|^2\delta_{ij}+
\frac{w^3}{4a_\text{max}\gamma^3}\fmax{s\in[0,1]}\|\ddot{I}(s)\|^2\delta_{ij}+\\
&\frac{w^4}{2a_\text{max}r^4}\frac{L_{\Delta t}^1}{L_{\Delta t}^2}\fmax{s\in[0,1]}\|\ddot{I}(s)\|+\frac{w^5}{8a_\text{max}^2r^5}\fmax{s\in[0,1]}\|\ddot{I}(s)\|^2\delta_{ij}.
\end{align*}
\normalsize
The result follows immediately.
\end{IEEEproof}
\begin{IEEEproof}[Proof of \prettyref{thm:LipDeltaT}]
Combining the result of \prettyref{lem:DeltaTA}, \prettyref{lem:DeltaTB}, and \prettyref{lem:DeltaTC}, we have:
\begin{align*}
&\left\|\FPPTT{\Delta t}{\bar{X}_i}{\bar{X}_j}\right\|_F
\leq\frac{L_{\Delta t}^1}{L_{\Delta t}^2}\frac{L_{\Delta t}^3+L_{\Delta t}^4\frac{2a_\text{max}\|\tilde{A}_j\|}{(a_\text{max}\Delta t^2-\|\tilde{A}_j\|)^2}}{L_{\Delta t}^2+\Theta}+\frac{L_{\Delta t}^5}{L_{\Delta t}^2}\\
\leq&\frac{L_{\Delta t}^1}{L_{\Delta t}^2}\frac{L_{\Delta t}^3+L_{\Delta t}^4\Theta}{L_{\Delta t}^2+\Theta}+\frac{L_{\Delta t}^5}{L_{\Delta t}^2}
\leq\frac{L_{\Delta t}^1}{L_{\Delta t}^2}(\frac{L_{\Delta t}^3}{L_{\Delta t}^2}+L_{\Delta t}^4)+\frac{L_{\Delta t}^5}{L_{\Delta t}^2},
\end{align*}
where we let $\Theta=\sum_i(2a_\text{max}\|\tilde{A}_i\|)/(a_\text{max}\Delta t^2-\|\tilde{A}_i\|)^2$, which might take any positive value. Since each block of Hessian matrix of $\Delta t$ is bounded by a constant independent of domain position, the result follows.
\end{IEEEproof}

==> old/convergenceADMM2.tex <==
\section{\label{sec:convADMM2}Convergence Analysis:\\ ADMM with Full Stiffness Decoupling}

==> old/fig4.tex <==
\begin{figure*}[ht]
\vspace{-5px}
\centering
\scalebox{0.8}{
%\includegraphics[width=.3\textwidth]{figs/indoor2.jpg}
%\includegraphics[width=.58\textwidth]{figs/b3d.jpg}
%\includegraphics[width=.8\textwidth]{single_uav.jpg}
\includegraphics[width=.64\textwidth]{bitmap.jpg}
%\includegraphics[width=.14\textwidth,trim=0cm -5.5cm 0cm -5.5cm,clip]{single_uav_initial.png}
%\includegraphics[width=.24\textwidth,trim=1.8cm 0.1cm 3.2cm 0.4cm,clip]{plot_hist.pdf}
%\includegraphics[width=.24\textwidth,trim=1.8cm 0.1cm 3.2cm 0.4cm,clip]{plot_hist.pdf}\llap{\makebox[\wd1][l]{\raisebox{1.9cm}{\includegraphics[width=.06\textwidth,trim=0cm -5.5cm 0cm -5.5cm,clip]{single_uav_initial.png}}}}
\def\big{\includegraphics[width=.33\textwidth,trim=1.8cm 0.1cm 3.2cm 0.4cm,clip]{plot_hist.pdf}}
\def\little{\includegraphics[width=.09\textwidth,trim=3.5cm -6.5cm 3.5cm -6.5cm,clip]{single_uav_initial.png}}
\stackinset{c}{15pt}{c}{24pt}{\little}{\big}
\put(-450,105){(a)}
\put(-425,10){(b)}
\put(-340,105){(c)}
\put(-330,10){(d)}
\put(-280,105){(f)}
\put(-195,5){(e)}
\put(-15,5){(g)}}
\vspace{-5px}
\caption{\label{fig:singleUAV}\small{Examples of trajectories generated by Safe-Corridor \cite{han2021fast} (blue) and ADMM \ref{alg:ADMM1} (red) for a single UAV in complex environments: indoor flight (a-c), outdoor flight (d-f). \revised{(g): The distributions of computational time of ADMM \ref{alg:ADMM1} and P-IPM \cite{2010.09904} over $600$ trajectories computed for a synthetic environment in which we compute $600$ random initial trajectories using RRT-connect.}}}
\vspace{-5px}
\end{figure*}

==> old/fig6.tex <==
\begin{figure*}[ht!]
%\vspace{-10px}
\centering
\scalebox{.8}{
\includegraphics[width=0.64\textwidth]{bitmap2.jpg}
%\includegraphics[width=.14\textwidth]{multi_hist.png}
%\includegraphics[width=.24\textwidth,trim=1.8cm 0.1cm 3.2cm 0.4cm,clip]{multi_hist.pdf}
\def\big{\includegraphics[width=.33\textwidth,trim=1.8cm 0.1cm 3.2cm 0.4cm,clip]{multi_hist.pdf}}
\def\little{\includegraphics[width=.12\textwidth]{multi_hist.png}}
\stackinset{c}{24pt}{c}{-4pt}{\little}{\big}
\put(-340,2){(a)}
\put(-180,2){(b)}
\put(-520,150){ADMM}
\put(-520,70){Penalty-Method \cite{zhou2020ego2}}
\put(-5,2){(c)}}
\vspace{-5px}
\caption{\label{fig:multiUAV}\small{Multiple UAV in complex environments, both with two groups of UAVs switching positions without (a) and with (b) obstacles. \revised{(c): The distributions of computational time of ADMM \ref{alg:ADMM1} and Penalty-Method \cite{zhou2020ego2} over $600$ trajectories computed for a synthetic environment in which we randomly generate initial trajectories for the $4$ UAVs in different homotopy classes.}}}
\vspace{-5px}
\end{figure*}

==> old/methodFull.tex <==
\begin{algorithm*}[ht]
\caption{\label{alg:ADMM2} ADMM with Full Stiffness Decoupling}
\small{\begin{algorithmic}[1]
\Require{$\theta^0,\bar{X}_i^0,\lambda_i^0,\TWO{n_i}{d_i}^0,\TWO{n_{ij}}{d_{ij}}^0$}
\For{$k=0,1,\cdots$}
\State $\theta^{k+1}\approx\argmin{\theta}\mathcal{L}(\theta,\bar{X}_i^k,\lambda_i^k,n_i^k,d_i^k,n_{ij}^k,d_{ij}^k)$\Comment{Update $\theta,\bar{X}_i,\lambda_i$}
\For{$i$th piece of trajectory}
\State $\bar{X}_i^{k+1}\approx\argmin{\bar{X}_i}\mathcal{L}(\theta^{k+1},\bar{X}_i,\lambda_i^k,n_i^k,d_i^k,n_{ij}^k,d_{ij}^k)+\frac{\varrho}{2}\|\bar{X}_i-\bar{X}_i^k\|^2$
\State $\lambda_i^{k+1}\gets\lambda_i^k+\varrho(X_i(\theta^{k+1})-\bar{X}_i^{k+1})$
\EndFor
\For{collision-free constraint between $i$th piece of trajectory and environment}\Comment{Optimize separating plane}
\State $\TWO{n_i}{d_i}^{k+1}\approx\argmin{\|n_i\|=1,d_i}\mathcal{L}(\theta^{k+1},\bar{X}_i^{k+1},\lambda_i^{k+1},n_i,d_i,n_{ij}^k,d_{ij}^k)$
\EndFor
\For{collision-free constraint between $i$th and $j$th piece of trajectory}
\State $\TWO{n_{ij}}{d_{ij}}^{k+1}\approx\argmin{\|n_{ij}\|=1,d_{ij}}\mathcal{L}(\theta^{k+1},\bar{X}_i^{k+1},\lambda_i^{k+1},n_i^{k+1},d_i^{k+1},n_{ij},d_{ij})$
\EndFor
\EndFor
\end{algorithmic}}
\end{algorithm*}
\subsection{ADMM with Full Stiffness Decoupling}
In the above section, we decoupled the objective function $\mathcal{O}$ from the log-barrier functions. However, the objective function for time-optimality, i.e., $w\Delta t$, is still coupled with velocity and acceleration limits. To achieve full stiffness decoupling, we plug slack variables $\bar{V}_i=\dot{I}\bar{X}_i$ and $\bar{A}_i=\ddot{I}\bar{X}_i$ into the velocity and acceleration limits of \prettyref{eq:ALF} and then consider the following $\Delta t$-subproblem:
\footnotesize
\begin{align*}
&\Delta t(\bar{X}_i)\triangleq\argmin{\Delta t}w\Delta t-\\
&\gamma\sum_{i}\log(v_\text{max}\Delta t-\sqrt{\|\bar{V}_i\|^2+\epsilon})-
\gamma\sum_{i}\log(a_\text{max}\Delta t^2-\sqrt{\|\bar{A}_i\|^2+\epsilon^2}),
\end{align*}
\normalsize
where we introduce a small, positive constant $\epsilon$ for regularization. Since the above subproblem is strictly convex in $\Delta t$, we can denote the result as a function $\Delta t(\bar{X}_i)$. Plugging this function back to \prettyref{eq:ALF} and we derive a reduced Lagrangian function of the following form:
\footnotesize
\begin{align*}
&\mathcal{L}(\theta,\bar{X}_i,\lambda_i,n_i,d_i,n_{ij},d_{ij})\triangleq\sum_i\mathcal{O}(\bar{X}_i)+w\Delta t(\bar{X}_i)+\\
&\gamma\sum_{i}\left[\sum_{x\in X_i}\log(n_ix(\theta)+d_i)+\sum_{z\in Z}\log(-n_iz-d_i)\right]-    \\
&\gamma\sum_{ij}\left[\sum_{x\in X_i}\log(n_{ij}x(\theta)+d_{ij})+\sum_{x\in X_j}\log(-n_{ij}x(\theta)-d_{ij})\right]+   \\
&\sum_i\frac{\varrho}{2}\|X_i(\theta)-\bar{X}_i\|^2+\lambda_i^T(X_i(\theta)-\bar{X}_i).\labelthis{eq:ALFF}
\end{align*}
\normalsize
We can ignore the log-barrier functions of velocity and acceleration limits because the function $\Delta t(\bar{X}_i)$ is guaranteed to satisfy the limits by construction. Our final ADMM \prettyref{alg:ADMM2} corresponds to finding the fixed points of \prettyref{eq:ALFF}, which achieves full stiffness decoupling. Indeed, the following lemma shows that $\Delta t(\bar{X}_i)$ is Lipschitz-continuous, so that $\mathcal{L}$ is Lipschitz-continuous in the $\bar{X}_i$-subproblem and log-barrier functions only appear in the $\theta$-subproblem:
\begin{lemma}
\label{lem:contDeltaT}
$\Delta t(\bar{X}_i)$ is smooth.
\end{lemma}
\begin{theorem}
\label{thm:LipDeltaT}
$\FPPR{\Delta t(\bar{X}_i)}{\bar{X}_i}$ is $L_{\Delta t}$-Lipschitz continuous for any point in the domain of $\bar{X}_i$.
\end{theorem}
We refer readers to \prettyref{sec:propertyDT} for their complete proof. Evaluating $\Delta t(\bar{X}_i)$ involves optimizing for a single variable $\Delta t$, which can be done efficiently using Newton's method. If $\Delta t(\bar{X}_i)$ is evaluated exactly during the update of $\bar{X}_i$ in \prettyref{alg:ADMM2}, then the convergence analysis of \prettyref{alg:ADMM2} is identical to that of \prettyref{alg:ADMM1}. This is because \prettyref{thm:LipDeltaT} shows that $\Delta t$ is a Lipschitz continuous function of $\bar{X}_i$ and can thus be absorbed into $\mathcal{O}$. In practice, however, we must terminate after finite number of iterations of Newton's method and the convergence analysis of \prettyref{alg:ADMM2} follows a similar argument as that of approximate bilevel optimization \cite{ghadimi2018approximation} with $\Delta$-subproblem being the strictly convex, low-level problem. We provide this proof at \prettyref{sec:convADMM2} for completeness.

==> old/old.tex <==
\begin{figure}[ht]
\vspace{-5px}
\centering
\includegraphics[width=.45\textwidth]{figs/placeholder.png}
\vspace{-5px}
\caption{\label{fig:ARM}\small{We command a set of 6-DOF UR10 robot arms' end-effectors to reach their respective target positions.}}
\vspace{-5px}
\end{figure}
\begin{figure}[ht]
\vspace{-5px}
\centering
\includegraphics[width=.235\textwidth]{figs/placeholder.png}
\includegraphics[width=.235\textwidth]{figs/placeholder.png}
\put(-228,10){(a)}
\put(-25,10){(b)}
\vspace{-5px}
\caption{\label{fig:ARMConv}\small{(a): Convergence history of partially decoupled ADMM, fully decoupled ADMM, and Newton-type method in terms of \#iterations and wall-time. (b): Convergence history of three algorithms plotted against the number of robot arms.}}
\vspace{-5px}
\end{figure}
\TE{Goal-Reaching of Multiple Robot-Arms:} As illustrated in \prettyref{fig:ARM}, we setup our simulator with multiple 6-DOF UR10 robot arms. Our objective is for each arm's end-effector $e(\theta)$ to reach a certain target position $e^*$ in a collision-free manner, i.e. $\mathcal{O}=\|e(\theta)-e^*\|^2$. Each link of the robot arm is discretized using a mesh and $x$ represents the Cartesian-space position vector of all the mesh vertices, while $\theta$ resides in the configuration space. The trajectory of an arm is approximately by piecewise linear discretization in configuration space, where velocities and accelerations are approximated using finite differences, i.e. $V_i\triangleq\theta_{i+1}-\theta_i$ and $A_i\triangleq\theta_{i+2}-2\theta_{i+1}+\theta_i$. The convergence history is summarized in \prettyref{fig:ARMConv} (a) and the change of computational time is plotted against the number of robot arms in \prettyref{fig:ARMConv} (b). Our method achieves up to $XXX\times$ speedup as compared with \cite{2010.09904} with a maximal number of $XXX$ robot arms.

\begin{figure}[ht]
\vspace{-5px}
\centering
\includegraphics[width=.45\textwidth]{figs/multi_uav2.png}
\vspace{-5px}
\caption{\label{fig:earlyStop}\small{Quality of trajectory (measured by total trajectory length) plotted against the number of iterations before termination.}}
\vspace{-5px}
\end{figure}
\ruiqi{do we keep this part?}
\TE{Online Trajectory Update:} Since constraints are always satisfied during an optimization, our algorithm can be terminated early at any iteration to account for various sources of uncertainty. We simulate this scenarios by controlling a group of $XXX$ UAVs to reach their target positions, i.e. $\mathcal{O}=\|e(x)-e^*\|^2$, in a receding horizon fashion. We optimize a short trajectory with $XXX$ B\'ezier curve pieces for each UAV, stop the optimization early after a certain number of iterations, and then have each UAV tracks the first B\'ezier curve. In \prettyref{fig:earlyStop}, we plot the quality of trajectories (measured by total trajectory length) against the number of iterations before termination, as compared with full optimization. Our method can achieve $XXX$Hertz of optimization within $XXX$ iterations without a significant loss of optimality.
